Online Object and Task Learning via Human Robot Interaction

This work describes the development of a robotic system that acquires knowledge incrementally through human interaction where new tools and motions are taught on the fly. The robotic system developed was one of the five finalists in the KUKA Innovation Award competition and demonstrated during the Hanover Messe 2018 in Germany. The main contributions of the system are a) a novel incremental object learning module - a deep learning based localization and recognition system - that allows a human to teach new objects to the robot, b) an intuitive user interface for specifying 3D motion task associated with the new object, c) a hybrid force-vision control module for performing compliant motion on an unstructured surface. This paper describes the implementation and integration of the main modules of the system and summarizes the lessons learned from the competition.

==> Text/abstract.tex <==
... 





\begin{comment}
This paper describes the ...


For some applications, imposing a virtual nonholonomic constraint (VNHC) on the motion of the end effector can help prevent operators from moving in an unintended direction by reducing
the number of controllable degrees of freedom. This paper presents the development of a VNHC for a planar time-delayed telerobotic task, motivated by an on-orbit telerobotic satellite



We also describe a nonholonomic virtual  fixture (NHVF) that adheres to the VNHC to further reduce the potential for operators to input mistaken commands.




servicing operation. We also

This paper introduces a manipulator robot surface
following algorithm using a 3D model of vehicle body panels
acquired by a network of rapid but low resolution RGB-D
sensors. The main objective of this work is to scan and
dynamically explore regions of interest over an automotive
vehicle body under visual guidance by closely following the
surface curves and maintaining close proximity to the object.
The work is motivated by applications in automated vehicles
inspection and screening in security applications. The proposed
path planning strategy is developed based on a perception modeling-planning-action
approach. Raw data rapidly
captured by a calibrated network of Kinect sensors are
processed to provide the required 3D surface shape of objects,
normal measurements, orientation estimation, and obstacle
detection. A robust motion planning method is designed that
relies on this information, resulting in a safe trajectory that is
planned to follow and explore the curved surfaces while
avoiding collision with protruding components of the vehicle.
The feasibility and effectiveness of the proposed method is
validated through experimental results with a 7-DOF
manipulator navigating over automotive body panels. 


he limited bandwidth of sensor-based feedback control restricts the execution speed of a force controlled planar contour following task, if the shape of the workpiece is unknown. This paper shows how appropriate feedforward control of the task frame orientation, calculated online from an eye-in-hand camera image, results in a higher quality (i.e. faster and/or more accurate) task execution. However, keeping the contour in the camera held of view in addition to maintaining a force controlled contact, imposes additional requirements on the controller. This double control problem is specified in the task frame formalism and executed in a hybrid position/force control environment. It is solved using the redundancy for the rotation in the plane, which exists for rotational symmetric tools. The key in this solution is (continuously) redefining the relation between the task frame and the end effector. Experimental results are presented to validate the approach.

In direct teleoperation, 
the users performance was better in bilateral configuration than
the unilateral configuration. In contrast,  our system
both bilateral and unilateral configuration obtain similar
performance, in terms of execution time of task, smoothness of path, 

\end{comment}



==> Text/detection.tex <==
possible applications are : welding , writing , sealing/gluing , icing of cake , cleaning , polishing (industry + home applications) ...

X-joint welding ... 
space related tasks: repairing, changing battery, .... 



==> Text/experiments.tex <==



The experiments consist of two main tasks: drawing on a surface and a circular alignment. Users are required to maintain the contact with the surface during the tasks. We conducted a pilot study with 9 users (2 female and 7 male). \kkk The tests were approved by University of Alberta Research Ethics and Managements (Pro00054665). \kkk
All of the users have normal or corrected to normal vision. 
The complete experiment took about 90 minutes per participant. For each task users utilize all 4 different system configurations described in section~\ref{sec:system_description}.  
The sequence of the tasks and the teleoperation configuration was randomized across participants.
At the end of the experiment the users were asked to fill a 21 scale NASA TLX form.

\begin{figure}[h]
\centering
\caption{Three different experiments were conducted using both direct teleoperation and our VF controller. From left to right: line drawing, path drawing and circular alignment tasks.}
\label{fig:experimental_setup}
\end{figure}

\kkk
\subsection{Controller Parameters}
The following controller gains are chosen for all the interface experiments. A nominal force of $F_0 = 4 \, N$ is applied for maintaining the contact. 
\begin{table}[h]
\begin{center}
\setlength{\tabcolsep}{5 pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{|l| c c | } \hline
    & Stiffness Gain & Damping Gain \\ \hline
Path Controller & 1000 & 10  \\ \hline
Normal Force Controller & 10 & 0.1 \\ \hline
Tangential Force Controller & 15 & 0.01 \\ \hline
Orientation Controller & diag(7,7,0) & 0.01*diag(1,1,1) \\ \hline
\multirow{2}{*}{Bilateral Controller} & diag(900, 2500,  600, & diag(10,20,5,2, \\
& 500,   50,   50,8) &   0.5,0.5,0.05)  \\ \hline
\end{tabular}
\end{center}
\caption{Controller gains}
\label{table_Controllers}
\end{table}
\subsection{Tasks Description}
\subsubsection{Drawing Task}
The participant is presented with two drawing patterns: a \textit{Line} (Fig.~\ref{fig:experimental_setup}A) and a sinusoidal \textit{Path} (Fig.~\ref{fig:experimental_setup}B). The drawing task consists of tele-operating the remote robot with a pen attached to its end-effector. Users have to make contact with the surface on one end of the pattern and follow it through without lifting the pen from the surface. To perform these tasks users first click on the image to define the desired path. Once defined, users manually activate the VFs  to constrain the robot to the path they defined.

\subsubsection{Circular Alignment Task}
A pattern with two arrows (green and red) is placed on top of a turntable as shown in Fig.~\ref{fig:experimental_setup}C. Initially, the red arrow is aligned with an orange marker. The task is then to align the green arrow with the marked location by rotating the turntable. To rotate the turntable, users have to make contact with the turntable first, and then maintain the contact while rotating in a counter-clockwise circular motion.

\kkk
\subsubsection{3D-writing on a Ball}
We demonstrate the capability of our proposed control architecture on a challenging task of following an arbitrary 3D path on a ball. Snapshots of the task are shown in Fig. \ref{fig:3D-task}. Demonstrations of these tasks can be seen in the attached video.   
\kkk



\subsection{Anecdotal Examples}

To proof the applicability of our interface to real world scenarios we complete two anecdotal examples: 1) Closing a steam vale. 2)  Gluing a T PVC pipe.

\subsubsection{Closing a steam valve}
As a proof of concept we run a test during a robot demonstration in an Industrial Mixer at the University of Alberta Computing
Science building. The task consists of closing a steam valve (see Fig.~\ref{fig:steam}) through teleoperating a 7-DOF robot located in the department's 2nd floor, 
with a 4-DOF WAM arm located in our robotics lab (department's 3rd floor). Through this task we show
the viability of using our system in a real task. We noticed that by planing the robot trajectory beforehand the task is carefully laid out and 
obstacles that were hit during direct teleoperation were avoided during the task specification 
(see the video attached).



\subsubsection{Gluing a T PVC pipe}

Our interface allows to specify different magnitudes of normal contact force to complete tasks like welding, polishing, painting, etc. which require moving through a specific path while making contact with a surface. In this example the objective is to apply glue to a crack on a PVC pipe, see Fig.~\ref{fig:tube_task}. 








\subsection{Results and Analysis}
While performing the task, the position and orientation of the remote robot was recorded for analysis. In addition, when using the interface  the points clicked by the user (hereafter referred to as \textit{interface path}) are recorded. 
Trajectories of the end-effector controlled by one of the participants are shown in Fig.~\ref{fig:traj-interfaces} for different tasks and with different teleop configurations. \kkk The red dashed-line represents the  ground truth path, which is obtained by moving the tip of the robot to the desired path and recording the pose. \kkk 
It is clear from Fig.~\ref{fig:traj-interfaces} that each teleop configuration presents a different characteristic behaviour in the tasks.
The following four metrics are used to characterize/evaluate the performance of teleop configurations.

\subsubsection{Path Smoothness}
The smoothness of each path was assessed using the \textit{Spectral Arc Length} (SAL) metric developed in \cite{smoothness_measure}. SAL is a dimensionless measure of the length of the frequency spectrum curve of a 
speed profile over the bandwidth appropriate for the motion. 
For a movement with speed profile $v(t)$, SAL is calculated from
$$SAL := \int_0^{\omega_c} \sqrt{ \big({\tfrac{1}{\omega_c}}\big)^2 + \big( { \tfrac{dV(\omega)}{d\omega} } \big)^2 } d\omega.$$
where $V(\omega)$ is the Fourier magnitude spectrum of $v(t)$, and
$[0,\omega_c ]$ is the frequency band spanned by the given movement. 
$\omega_c = 40 \pi$ rad/s (which corresponds to 20 Hz) covers the normal
and abnormal aspects of human movements \cite{smoothness_measure}. 
It should be noted that SAL value approaches zero with increases in smoothness of the path. 

Figure \ref{fig:smoothness_compare} (top) compares the smoothness of the paths for different teleop configurations and for different tasks. It can be seen from this figure that  VF improves the smoothness of the paths. \kkk As expected, game-pad teleop configuration results in the most jerky (non-smooth) motions. Adding the virtual fixtures significantly improves the smoothness of the paths.  In fact, the smoothness of the paths with uni-VF configuration is (on the average) better than bilateral configuration and comparable with bilateral with VF configuration. This is due the fact that in uni-VF mode, the operator is only able to move the robot along the path. \kkk


\subsubsection{Time to complete the task}
Figure \ref{fig:smoothness_compare} (bottom) compares the execution time of each task for different teleop configurations. 
Note that the time to set the path from the interface is not considered here in the measurements as this procedure can be done offline.
It can be seen from this figure that VF reduces the execution time of  the tasks in unilateral configuration.  \kkk Uni-VF performed the best as anticipated; adding a driving force in the tangential direction helps the operator to finish the task faster. \kkk



\subsubsection{Trajectory Error}

Table \ref{table1} presents the trajectory mean error (averaged over all participants) for the line and sinusoidal paths. \kkk Given the ground truth path ($\bm P_{GT}$), the  error from the path is computed as the minimum distance of the sampled trajectory to the path, \textit{i.e.} 
$ e( \bm x)  = \min_{\bm p \in \bm P_{GT} } \| \bm x - \bm p \|$. \kkk
\kkk It can be seen from Table \ref{table1} that the bi-VF has the best performance in terms of trajectory following. While the performance of the unilateral teleop is not satisfactory,  adding the VF significantly improve the performance of the uni-VF teleop up to a point that is comparable to bi-VF. Note that the error in the bilateral configuration is higher compared to  uni-VF control. 
This observation is in line with the one of \cite{castillocruces2009},  
because in  bilateral mode, operator has to control both position and orientation simultaneously. 
Authors of \cite{castillocruces2009} stated that this is due to the translational and rotational components of motion being decoupled from each other in such a way that the user, focusing on moving one, will not notice an error in the other and vice versa.  
The same trend is observed in the variance of the errors, except that the variance of the error is smaller for the uni-VF. This could be due the fact that in the uni-VF mode, the operator is only able to move along the path direction. In the bi-VF mode, however the operator is able to fight with VF and move in other directions. 
\kkk
\begin{table}[h]
\begin{center}
\setlength{\tabcolsep}{5 pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{|lr|c c c c | } \hline
\multicolumn{2}{|c|}{}                    & uni & bi  & uni-VF  & bi-VF \\ \hline
\multirow{2}{*}{Line} & mean error (mm)  & 13.78  & 11.76  & 4.50 & \textbf{4.37}    \\ 
    & variance (mm)  & 8.15 &	5.96  &	\textbf{1.52} &	2.19     \\ \hline
\multirow{2}{*}{Path} & mean error (mm)  &  13.99    & 11.13  & 9.08 & \textbf{8.51}    \\ 
    & variance (mm) & 9.58    &	7.53  &	\textbf{4.07} &	3.42    \\ \hline
\end{tabular}
\end{center}
\caption{Comparison of the trajectory error and variance for different teleop configurations}
\label{table1}
\end{table}

\subsubsection{Loss of Contact}
Table  \ref{table2}  compares the average number of times that the robot's end-effector tip lose the contact with the surface during the experiments. In the simple uni-lateral control, it is hard for the operator to maintain the contact with the environment due to the lack of haptic feedback through the game-pad.  Contact control improves in the bilateral case as the user is able to feel the force feedback from the remote site and tries to maintain the contact. Table \ref{table2} shows the effectiveness of the normal force controller in maintaining the contact with the environment. 
\kkk
\begin{table}[h]
\begin{center}
\setlength{\tabcolsep}{5 pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{|l|c c c c | } \hline
        & uni & bi  & uni-VF  & bi-VF \\ \hline
Line    & 2.71  & 0.75 & 0 & 0        \\ \hline
Path    & 3.33  & 1.14 & 0.28 & 0     \\ \hline
\end{tabular}
\end{center}
\caption{Average number of loss of contact with the surface during the line /path following tasks}
\label{table2}
\end{table}
\kkk

In summary, the the performance of the unilateral with VF in terms of error, execution time, smoothness of the path and contact control is comparable to the one of bilateral control with VF. This also signifies that lack of haptic feedback in the unilateral control can be compensated by proper integration of vision and force control.

\subsubsection{Operator Workload Measure}
Figure \ref{fig:TLX} shows the mean ratings of each workload category reported by the users in the NASA TLX survey. 
The uni-VF configuration resulted in less overall workload than all the other configurations including the bi-VF. This again confirms our hypothesis that by
introducing  vision-force assistive constraints, the operator's performance in the unilateral case can be improved, perhaps up to the point where performance is similar to the bilateral configuration.
\begin{figure}[h]
\centering
\includegraphics[width=.4\textwidth] {figures/NASA_TLX.eps}
\caption{Nasa TLX radar plot: Qualitative workload evaluation, higher workloads are farther from the center of plot.}
\label{fig:TLX}
\end{figure}








\begin{comment}




\kkk 3D task \kkk

A- tele-op with joystick



B- tele-op with haptic feedback

-- ) only tele-op without assistive visual/force fixtures

-- ) tele-op with assistive visual/force fixtures 


\rrr 
 the metrics are : -1 smoothness of the path , 2) the time to complete the task, 3) the error, 

 experiment variables: 1) remote device ( joy-stick = non-symmetric config. , wam - wam = sym. config.) 
                        2) delay
                        3) force / no-force ( contact  force feedback) 
                        4) Visual Fixture / No VF (with only visual feedback ) 
                        5) user velocity

                        
=> the conclusion : hypothesis is that non-sym tele-op with assistive VF will have the similar performance of the sym configuration with visual/force assist 
while non-sym tele-op is worse than the sym teleop  without the VF.
\kkk 


\rrr 
Future work: 
Consider the effect of friction, model of the friction force to compensate for it.  

\kkk



\begin{figure}[h]
\centering
\includegraphics[trim=23mm 0mm 1mm 7mm, clip=true, width=.3\textwidth] {figures/line_VFT_biVF_compare.eps}
\caption{Comparison of line following with uni-VF-T interfaces and bi-VF}
\label{fig:VFT_results}
\end{figure}


\end{comment}













